Some Best Practices in Operator Learning

Hyperparameters searches are computationally expensive. This paper studies some general choices of hyperparameters and training methods specifically for operator learning. It considers the architectures DeepONets, Fourier neural operators and Koopman autoencoders for several differential equations to find robust trends. Some options considered are activation functions, dropout and stochastic weight averaging.

==> precision.tex <==
\section{Precision}

The precision\index{precision} of the input and the weights of the model can vary. In this section, using $16$-bit precision, $32$-bit precision and $64$-bit precision are compared. 
Using a lower precision can accelerate teh training of the model \cite{gupta2015deep, henry2019leveraging, tu2023guaranteed}. 
But, using a lower precision can also decrease the accuracy of the model.
Furthermore, the number of bits used for the mantissa for matrix multiplication can very. The \emph{highest}\index{highest} precision uses a $24$-bit mantissa, the \emph{high}\index{high} precision uses a $11$-bit mantissa and the \emph{medium}\index{medium} precision uses a $8$-bit mantissa. 

% Experiment paragraph


\begin{table}[H]
    \caption{Results for precision: The left table is for a Koopman autoencoder for the equation for the pendulum. The center table is for a DeepONet for Burger's equation. The right table is for a Fourier neural operator for the KdV equation.}
    \label{precision}
    \begin{minipage}{.32\textwidth}
        \vspace{1em}
        \begin{center}
        Koopman and pendulum \\
        \begin{tabular}{lr}
            error & precision \\
            \toprule
            4.185e-4 & 16-bit \\
            3.681e-4 & 32-bit \\
            5.559e-4 & 64-bit \\
        \end{tabular}
        \end{center}
    \end{minipage}
    \begin{minipage}{.32\textwidth}
        \vspace{1em}
        \begin{center}
        DeepONet and Burger's \\
        \begin{tabular}{lr}
            error & precision \\
            \toprule
            3.328e-3 & 16-bit \\
            4.081e-3 & 32-bit \\
            3.504e-3 & 64-bit \\
        \end{tabular}
        \end{center}
    \end{minipage}
    \begin{minipage}{.32\textwidth}
        \vspace{1em}
        \begin{center}
        FNO and KdV \\
        \begin{tabular}{lr}
            error & precision \\
            \toprule
            & 16-bit \\
            & 32-bit \\
            & 64-bit \\
        \end{tabular}
        \end{center}
    \end{minipage}
\end{table}

\begin{table}[H]
    \caption{Results for the precision of matrix multiplication: The left table is for a Koopman autoencoder for the equation for the pendulum. The center table is for a DeepONet for Burger's equation. The right table is for a Fourier neural operator for the KdV equation.}
    \label{matmul}
    \begin{minipage}{.32\textwidth}
        \vspace{1em}
        \begin{center}
        Koopman and pendulum \\
        \begin{tabular}{ll}
            error & precision \\
            \toprule
            9.652e-5 & medium \\
            2.156e-4 & high \\
            6.905e-4 & highest \\
        \end{tabular}
        \end{center}
    \end{minipage}
    \begin{minipage}{.32\textwidth}
        \vspace{1em}
        \begin{center}
        DeepONet and Burger's \\
        \begin{tabular}{ll}
            error & precision \\
            \toprule
            0.00363181 & medium \\
            0.00323892 & high \\
            0.00300861 & highest \\
        \end{tabular}
        \end{center}
    \end{minipage}
    \begin{minipage}{.32\textwidth}
        \vspace{1em}
        \begin{center}
        FNO and KdV \\
        \begin{tabular}{ll}
            error & precision \\
            \toprule
            & medium \\
            & high \\
            & higest \\
        \end{tabular}
        \end{center}
    \end{minipage}
\end{table}


% Conclusion paragraph
% It is common that a lower precision can lead to instability in training. 

\section{Conclusion}

For operator learning, it recommended to use $\mathrm{gelu}$ as the activation function. 
It is recommended to not use dropout. 
It is recommended to use stochastic weight averaging with a learning rate that is not bigger than the original learning rate. 
And, it is recommended to not use a learning rate finder, but instead find it when hyperparameter tuning. 

